Plenoptic PNG: Real-Time Neural Radiance Fields in 150 KB

The goal of this paper is to encode a 3D scene into an extremely compact representation from 2D images and to enable its transmittance, decoding and rendering in real-time across various platforms. Despite the progress in NeRFs and Gaussian Splats, their large model size and specialized renderers make it challenging to distribute free-viewpoint 3D content as easily as images. To address this, we have designed a novel 3D representation that encodes the plenoptic function into sinusoidal function indexed dense volumes. This approach facilitates feature sharing across different locations, improving compactness over traditional spatial voxels. The memory footprint of the dense 3D feature grid can be further reduced using spatial decomposition techniques. This design combines the strengths of spatial hashing functions and voxel decomposition, resulting in a model size as small as 150 KB for each 3D scene. Moreover, PPNG features a lightweight rendering pipeline with only 300 lines of code that decodes its representation into standard GL textures and fragment shaders. This enables real-time rendering using the traditional GL pipeline, ensuring universal compatibility and efficiency across various platforms without additional dependencies.

==> figures/highlight.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/highlight_v0.pdf}
    \caption{\textbf{Examples of 3D scene files produced by \method:} TBA}
    \label{fig:overview}
\end{figure*}

==> figures/method.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/metphod_v0.pdf}
    \caption{\textbf{Overview of \method:} TBA}
    \label{fig:overview}
\end{figure*}

==> figures/realtime_demo.tex <==


\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{images/figures/phone_edited.jpg}
    \caption{
        We visualize all scenes in Synthetic NeRF dataset using PPNG-1. 
        The rendered scenes are from single screenshot captured from a phone (Apple iPhone 11 Pro Max.) \todo{could we also show a collection of iPad / MacBook / desktop? current aspect ratio wastes space and is iPhone only. }}
    \label{fig:phone}
\end{figure}

==> tex/method_12.tex <==
\section{Plenoptic PNG}
The goal of PPNG is to encode a set of images with known poses into a small model that can be efficiently transmitted and rendered on ubiquitous devices. To achieve this, we first formulate a representation (PPNG-3) that can be rendered efficiently and then formulate factorized representations (PPNG-1, PPNG-2) that are more compact, directly trainable, and efficiently composable after transmission into PPNG-3 for rendering. We implement the models in \textit{tiny-cuda-nn} to support fast training using a voxel-based density cache~\cite{Mller2022InstantNG}, and provide GLSL based code to decode the weights for real-time rendering. 

\subsection{3D Radiance Field Representation with PPNG-3}
\label{ssec:ppng-3}
Our PPNG-3 representation (Figure~\ref{fig:ppng3}) draws insight from the multi-resolution sinusoidal design of positional encoding functions~\cite{tancik2020_fourier}. But, rather than inputting the encodings vectors into a many-layer network, we use them to interpolate into multi-resolution periodic feature volumes, and the resulting feature vector is input into a shallow MLP  $f_{\btheta}(\cdot)$. Compared to deep MLPs, the feature volumes are faster to train, and the feature interpolation and shallow MLP are efficiently performed using standard web-based libraries. PPNG-3 encodes query point $\bx \in \mathbb{R}^3$ as :
\begin{align*}
    \gamma(x_k) &= [\sin(2^{0\ldots L-1}\pi x_k), \cos(2^{0\ldots L-1}\pi x_k)] \\
    \gamma(\bx) &= \text{concat}([\gamma(x_0),\gamma(x_1),\gamma(x_2)]) \in \mathbb{R}^{(2 \times L) \times 3}
\end{align*}

Given $2 \times L$ values for sinusoidal encodings of $\bx$, we trilinearly interpolate into $2 \times L$ number of 3D feature volumes $\bphi = \{\phi^{sin}_0, … \phi^{cos}_{L-1}\}$ of channel size $C$ (indexed from -1 to 1):
\begin{align*}
    \tau(\bx; \bphi)_i = \text{interp}(\gamma(x_0)_i, \gamma(x_1)_i, \gamma(x_2)_i, \bphi_{i})
\end{align*}
We aggregate the interpolated features of all spectrum, for each frequency of length $L$, and for each sines and cosines.
The resulting feature vector of length $F = 2 \times L \times C$, is passed into a shallow MLP $f_{\btheta}$ to regress density $\mathbf{\sigma}$ and appended with encoded viewing direction to regress color $\mathbf{c}$. 

\input{figures/ppng_1_and_2}
\subsection{Compact Plenoptic Representation with PPNG-1,2}
\label{ssec:ppng-12}
The number of parameters in PPNG-3 is $(F \times Q^3) + \|f_\btheta \|$, where Q represents quantization of 3D feature volume. This makes it hard to reduce the model size without significantly sacrificing quality by reducing Q. Since our volumetric representation is axis aligned, we use volume decomposition techniques to further compress the model size, similar to~\cite{Chen2022TensoRFTR}. 

To compress the 3D feature volume of PPNG-3, we use two types of decomposition: (1) tensor-rank~(CP) decomposition which decomposes 3D volumes into set of $R_{1}$ triplets of 1D vectors (denoted as PPNG-1), and (2) Tri-plane decomposition which decomposes 3D volumes into set of $R_{2}$ triplets of 2D vectors (denoted as PPNG-2). We visualize these decompositions in Figure~\ref{fig:ppng_1_2}.

For each feature volume $\bphi_i \in \mathbb{R}^{C \times Q^3}$ in PPNG-3 volumes, we define corresponding CP-decomposed PPNG-1 vectors $v^r_x, v^r_y, v^r_z \in R^{C \times Q}$ with $ 1 \leq r \leq R_1$ as:
\begin{align*}
    \bphi_i = \sum_{1 \leq r \leq R_1} v^r_x \cdot  v^r_y \cdot  v^r_z
\end{align*}
Similarly, we define corresponding tri-plane decomposed PPNG-2 planes $P^r_{x,y}, P^r_{y,z}, P^r_{x,z} \in R^{C \times Q \times Q}$ with $ 1 \leq r \leq R_2$ as:
\begin{align*}
    \bphi_i = \sum_{1 \leq r \leq R_2} P^r_{x, y} \cdot  P^r_{y, z} \cdot  P^r_{x, z}
\end{align*}
Note that computation of PPNG-3 from PPNG-1 and PPNG-2 is trivially parallelizable, each taking compute complexity of $\mathbb{O}(Q^3 \times R_1)$ and $\mathbb{O}(Q^3 \times R_2)$ respectively. 
After decomposition, PPNG-1 compresses PPNG-3 by a factor of $\frac{3 \times R_1}{Q^2}$ and PPNG-2 compresses PPNG-3 by a factor of $\frac{3 \times R_2}{Q}$. 


==> tex/method_12_bk.tex <==
\section{Plenoptic PNG}
The goal of PPNG is to encode a set of images with known poses into a small model that can be efficiently transmitted and rendered on ubiquitous devices. To achieve this, we first formulate a representation (PPNG-3) that can be rendered efficiently and then formulate factorized representations (PPNG-1, PPNG-2) that are more compact, directly trainable, and efficiently composable after transmission into PPNG-3 for rendering. We implement the models in \textit{tiny-cuda-nn} to support fast training using a voxel-based density cache~\cite{Mller2022InstantNG}, and provide GLSL based code to decode the weights for real-time rendering. 

\subsection{3D Radiance Field Representation with PPNG-3}
\label{ssec:ppng-3}
Our PPNG-3 representation (Figure~\ref{fig:ppng3}) draws insight from the multi-resolution sinusoidal design of positional encoding functions~\cite{tancik2020_fourier}. But, rather than inputting the encodings vectors into a many-layer network, we use them to interpolate into multi-resolution periodic feature volumes, and the resulting feature vector is input into a shallow MLP $f_{\btheta}$. Compared to deep MLPs, the feature volumes are faster to train, and the feature interpolation and shallow MLP are efficiently performed using standard web-based libraries. 

PPNG-3 encodes query point $\mathbf{p}=(x, y, z) \in \mathbb{R}^3$ as :
\begin{align*}
    \gamma(p) = [&(sin(f_1 x), sin(f_1 y), sin(f_1 z)), \\
                 &(cos(f_1 x), cos(f_1 y), cos(f_1 z)), \\
                 & … \\
                 &(sin(f_L x), sin(f_L y), sin(f_L z)), \\
                 &(cos(f_L x), cos(f_L y), cos(f_L z))] \in \mathbb{R}^{(2 \times L) \times 3}
\end{align*}
Given $2 \times L$ values for sinusoidal encodings of $(x, y, z)$, we trilinearly interpolate into $2 \times L$ number of 3D feature volumes $\mathbf{V} = \{V^{sin}_1, … V^{cos}_L \}$ with each volume shapes as $C \times Q^3$ of channel size $C$ and voxel resolution $Q$.



The resulting feature vector of length $F = 2 \times L \times C$, is passed into a shallow MLP $f_{\btheta}$ to regress density and geometric features, which are appended with encoded viewing direction to regress color. 


\input{figures/ppng_1_and_2}
\subsection{Compact Plenoptic Representation with PPNG-1,2}
\label{ssec:ppng-12}
The number of parameters in PPNG-3 is $(F \times Q^3) + \|\theta\|$, where Q represents quantization of 3D feature volume. This makes it hard to reduce the model size without significantly sacrificing quality by reducing Q. Since our volumetric representation is axis aligned, we use volume decomposition techniques to further compress the model size, similar to~\cite{Chen2022TensoRFTR}. 

To compress the 3D feature volume of PPNG-3, we use two types of decomposition: (1) CP-decomposition which decomposes 3D volumes into set of $R_{1}$ triplets of 1D vectors (denoted as PPNG-1), and (2) Tri-plane decomposition which decomposes 3D volumes into set of $R_{2}$ triplets of 2D vectors (denoted as PPNG-2). 

For each volume $V$ in PPNG-3 volumes $\mathbf{V}$ indexed by $(i,j,k)$, we define corresponding CP-decomposed PPNG-1 vectors $v^r_x, v^r_y, v^r_z \in R^{C \times Q}$ with $ 1 \leq r \leq R_1$.
We then, can compose PPNG-3 from PPNG-1 as:
\begin{equation}
    V(i,j,k) = \sum_{1 \leq r \leq R_1} v^r_x(i) \cdot  v^r_y(j) \cdot  v^r_z(k)
    \label{eq:ppng_1_to_3}
\end{equation}
Similarly, we define corresponding tri-plane decomposed PPNG-2 planes $P^r_{xy}, P^r_{yz}, P^r_{xz} \in R^{C\times Q \times Q}$ with $ 1 \leq r \leq R_2$, and compose PPNG-3 as:
\begin{equation}
    V(i,j,k) = \sum_{1 \leq r \leq R_2} P^r_{xy}(i,j) \cdot  P^r_{yz}(j,k) \cdot  P^r_{xz}(i,k)
    \label{eq:ppng_2_to_3}
\end{equation}
Note that computation of PPNG-3 from PPNG-1 and PPNG-2 is trivially parallelizable, each taking compute complexity of $\mathbb{O}(Q^3 \times R_1)$ and $\mathbb{O}(Q^3 \times R_2)$ respectively. 
After decomposition, PPNG-1 compresses PPNG-3 by a factor of $\frac{3 \times R_1}{Q^2}$ and PPNG-2 compresses PPNG-3 by a factor of $\frac{3 \times R_2}{Q}$. 


==> tex/method_34.tex <==
\subsection{Encoding and Implementation Details}
For training, we implement PPNG-1, 2 and 3 in \textit{tiny-cuda-nn}~\cite{Mller2022tinycudann}, which supports voxel-based density caching~\cite{Mller2022InstantNG} for accelerated ray integration.
We set $Q=80$, $R_1=8$, $R_2=2$, $L=4$ and $C=4$ throughout all implementations. 

Our shallow MLP consists of 2 parts. 
The first part takes feature vector size of $F= 32 = 2 \times L \times C$, and produces density value, and geometric feature vector of length 15. We use 1 layer (i.e, no hidden layers) for the first part of shallow MLP. In ablation studies, we experiment with different number of layers. 
The second part takes viewing direction, which is encoded by spherical harmonics of degree 3 (which yields vector length of 16), geometric feature vector of length 15, and density value, which totals to input vector size of 32. The second part of shallow MLP contains one hidden layer of size 16, and outputs color value. In total, our shallow MLP contains 1072 parameters. 

With the chosen parameters, we have parameter size of $125 KB$ for PPNG-1, $2.45 MB$ for PPNG-2 and $32.7 MB$ for PPNG-3 using half-precision floating points (including shallow MLP weights). 
We encode voxel-based density cache using run-length encoding~(RLE). This typically results in $50 KB$ to $150 KB$ depending on the complexity of the scene. 
We use CBOR~\cite{Bormann2013ConciseBO} to aggregate the Fourier feature parameters, shallow MLP weights and the voxel-based density caches into a single binary file. We emphasize that there are \textbf{no additional processes} (a.k.a baking) in converting the optimized PPNG into a binary encoding. 

\subsection{Real-time Interactive and Portable Viewing}
We visualize PPNG representations in real-time by porting the volume rendering of PPNG in traditional GL pipeline using WebGL 2 with GLSL. Figure~\ref{fig:rendering} illustrates this process. 
Given binary PPNG file, we first check which PPNG type (among PPNG-1, 2 and 3) that the binary file contains. 
If the given binary is PPNG-1 or PPNG-2, we efficiently convert it to PPNG-3 using Eq~\ref{eq:ppng_1_to_3} or Eq~\ref{eq:ppng_2_to_3} respectively. The conversion is parallelized with GLSL based code. 

Given PPNG-3, we load each volumetric Fourier features $V$ as 3D texture images. Since we set $C = 4$, we can use texture format set as RGBA to load each volume into single 3D texture image. We set texture filtering parameter set to linear, which enables tri-linear interpolation for texture sampling the loaded volumes in GLSL.  
We then load RLE encoded voxel-based density cache for empty-space skipping, by decoding it as occupancy grid. 
Similar to the volumetric Fourier feature volumes, we load the occupancy grid as another single-channel 3D texture image. 
Finally, we load shallow MLP by chunking the MLP into set of 4x4 matrices (\texttt{Mat4}) for faster inference. 

At render time, we use fragment shader to perform volume rendering. From the camera origin, we cast ray to each pixel in world space, and densely sample along the ray. For each sample, we check if it is occupied with the occupancy grid. If occupied, we query density and color at the sampled point using method described in Subsection~\ref{ssec:ppng-3}. The sampled color and density are integrated with volume rendering equation~\cite{Mildenhall2020NeRFRS} and are terminated if accumulated transmittance falls below threshold. 

We include a GLSL implementation in the supplementary material. \jae{leaving mark for supp.}

==> tex/method_3dv.tex <==
\section{Plenoptic Portable Neural Graphics}
The goal of PPNG is to encode a set of images with known poses into a small model that can be efficiently transmitted and rendered on ubiquitous devices.

To achieve this, we builds on the key intuition that, like multi-resolutional hash encoding~\cite{Mller2022InstantNG}, multi-frequency sinusoidal encoding places the input coordinate at multiple resolutions in the restricted space of -1 to 1 (for hashing, it will be 1 to N = hash size). 

Unlike hash encoding, which loses neighborhood information due to randomized discrete indexing, sine and cosine functions preserve local neighborhoods. 
Hence, these representations can be quantized into a lattice structures (since adjacency order is preserved), such as voxel grids, and further decomposed into lower-level tensors, allowing extreme compressibility.

% \vspace{-3mm}
\subsection{Plenoptic Portable Neural Graphics}
\label{ssec:ppng}
Our core contribution lies in a novel volumetric neural feature representation referred to as plenoptic portable neural graphics. The goal of this learnable representation is to approximate the mapping from coordinates $\mathbf{p} \in \mathbb{R}^K$ to color and opacity values $(\mathbf{c}, \sigma) \in \mathbb{R}^{3+1}$.

\noindent\textbf{Positional Encoding}.
Following the success of coordinate-based neural networks, given the input query point $\mathbf{p}=(x, y, z)$, positional encoding~\cite{Mildenhall2020NeRFRS, tancik2020_fourier} is applied to map the Euclidean coordinates input to sinusoidal activations across $L$ different frequency levels for each axis: 

\vspace{-3mm}
\begin{equation}
\label{eq:pos_enc}
    \gamma(\mathbf{p}) = \text{concat}([\gamma(x), \gamma(y), \gamma(z)]) \in \mathbb{R}^{3\times L \times 2},
\end{equation}

where activation for each axis is 
\begin{align*}
\label{eq:pos_enc}
 \gamma(x) &= [(\sin(2^i\pi x), \cos(2^i\pi x))]_{i=0}^{L-1} \in \mathbb{R}^{L\times 2}, \\
 \gamma(y) &= [(\sin(2^i\pi y), \cos(2^i\pi y))]_{i=0}^{L-1} \in \mathbb{R}^{L\times 2}, \\
 \gamma(z) &= [(\sin(2^i\pi z), \cos(2^i\pi z))]_{i=0}^{L-1} \in \mathbb{R}^{L\times 2},
\end{align*}
% $\gamma(x) = [(\sin(2^i\pi x), \cos(2^i\pi x))]_{i=0}^{L-1}$, $\gamma(y) = [(\sin(2^i\pi y), \cos(2^i\pi y))]_{i=0}^{L-1}$, $\gamma(z) = [(\sin(2^i\pi z), \cos(2^i\pi z))]_{i=0}^{L-1}$. 
This resulting encoding is a continuous, multi-scale, periodic representation of $\mathbf{p}$ along each coordinate.  

\input{figures/ppng_1_and_2}

% $\gamma(\mathbf{p}) = \text{concat}([\gamma(x), \gamma(y), \gamma(z)]) \in \mathbb{R}^{3\times L \times 2}$ 


\noindent\textbf{Background}.~
NeRF~\cite{Mildenhall2020NeRFRS} leverages a deep MLP network $f_{\btheta}$ to predict color and opacity $(\mathbf{c}, \sigma) = f_{\btheta}(\gamma(\mathbf{p}))$, requiring millions of network inferences and thus resulting in slow rendering. An alternative is to store a dense, spatially-indexed feature volume $\mathbf{V} \in \mathbb{R}^{S^3 \times D}$, allowing for the direct querying of spatial features from the volume using the spatial coordinate $\mathbf{z} = \pi(\mathbf{p}, \mathbf{V}) \in \mathbb{R}^D$, where $\pi(\cdot, \cdot)$ denotes position based feature query, which can be a trilinear interpolation~\cite{Liu2020NeuralSV}, spatial hashing function~\cite{Mller2022InstantNG}, or tri-plane interpolation~\cite{Chen2022TensoRFTR}. The feature can either be directly color and opacity~\cite{Yu2021PlenoxelsRF}, or a learned feature that is sent to a shallow decoder network~\cite{Liu2020NeuralSV, Mller2022InstantNG}. Although spatial feature volume is fast due to the efficiency of trilinear feature interpolation, it often results in a relatively large size.

\noindent\textbf{Fourier-indexed Feature Representation}.~
We develop an efficient and compact representation % to combine the best of two worlds, implicit modeling and feature volume query: 
that leverages: (1) positional encoding to convert the spatial coordinate into a multi-scale, multi-dimensional Fourier embedding; and (2) volume-based feature queries to enable fast inference. Specifically, we maintain $L\times 2$ feature volumes $\mathbf{V}^\mathrm{sin}_{i}, \mathbf{V}^\mathrm{cos}_{i} \in \mathbb{R}^{Q^3 \times D}$, each of which is a 3D feature volume, indexed by a 3D slice of the positional encoding $\gamma_i^\mathrm{sin} = [\sin(2^i\pi x),$ $ \sin(2^i\pi y), \sin(2^i\pi z)]$ (or cosine embedding $\gamma_i^\mathrm{cos}$).

\noindent\textbf{Inference}.~
During the inference, given a query point $\mathbf{p}$, we first compute the positional embedding $\gamma(\mathbf{p})$ using Equation~\ref{eq:pos_enc}. 
We then query feature vector $\mathbf{z}^\mathrm{sin}_i, \mathbf{z}^\mathrm{cos}_i$ from each volume across each frequency: 
\begin{equation}
\label{eq:query}
\forall i:  \text{\ } \mathbf{z}^\mathrm{sin}_i =  \pi_\mathrm{trilinear}(\gamma_i^\mathrm{sin}, \mathbf{V}_i^\mathrm{sin}), \text{\ }
  \mathbf{z}^\mathrm{cos}_i = \pi_\mathrm{trilinear}(\gamma_i^\mathrm{cos}, \mathbf{V}_i^\mathrm{cos})
\end{equation}
where $\pi_\mathrm{trilinear}$ is trilinear interpolation. 
We then concat all the features $\mathbf{z}(\mathbf{p}) = \mathrm{concat}[...\mathbf{z}^\mathrm{sin}_i, \mathbf{z}^\mathrm{cos}_i...]_{i=0}^L$, which result in a feature vector of length $F = 2 \times L \times D$. Finally, this feature vector is passed into a shallow MLP $f_{\btheta}$ with encoded viewing direction $\mathbf{d}$ to regress opacity and view-dependent color: 
\begin{equation}
    (\mathbf{c}, \sigma) = f_{\btheta}(\mathbf{z}(\mathbf{p}), \mathbf{d})
\end{equation}

\noindent\textbf{Remark}.~Despite its simplicity, our design offers multiple benefits. {\it Efficiency:} Similar to volume-based neural fields, our approach is extremely efficient, enabling real-time rendering. {\it Feature sharing:} Features at each voxel location in the Fourier domain are shared and accessed simultaneously by multiple spatial locations. This design allows us to extract redundancies over space (compared to spatial volumes) while maintaining smoothness (unlike spatial hashing). {\it Compactness:} The total model size is $L \times 2 \times Q^3 \times D + |\btheta|$, where $|\btheta|$ represents the number of parameters for the shallow MLP. In practice, given the redundancies and the multi-scale nature of each volume, the size of each volume $Q$ can be significantly smaller than the typical size for spatial volumes $S$ (e.g. 80 vs 512), resulting in a smaller overall model size.


% Then, $\bv$ is computed as:
% \begin{equation}
% \bv = f_{\btheta}(\gamma(\bx))%: \bbR^3 \rightarrow \bbR^D
% \end{equation}
% Given each query point $\mathbf{p}=(x, y, z)$, we encode into sinusoidal positional encoding
% \begin{equation}
%     \boldsymbol{\phi}(\mathbf{p}) = [...\phi_x^k, \phi_y^k, \phi_z^k...]
% \end{equation}
% % \begin{equation}
% %     \mathbf{V}[]
% % \end{equation}

% \subsection{3D Radiance Field Representation with PPNG-3}
% \label{ssec:ppng-3}
% Our PPNG-3 representation (Figure~\ref{fig:ppng3}) draws insight from the multi-resolution sinusoidal design of positional encoding functions~\cite{tancik2020_fourier}. But, rather than inputting the encodings vectors into a many-layer network, we use them to interpolate into multi-resolution periodic feature volumes, and the resulting feature vector is input into a shallow MLP $f_{\btheta}$. Compared to deep MLPs, the feature volumes are faster to train, and the feature interpolation and shallow MLP are efficiently performed using standard web-based libraries. 

% PPNG-3 encodes query point $\mathbf{p}=(x, y, z) \in \mathbb{R}^3$ as :
% \begin{align*}
%     \gamma(p) = [&(sin(f_1 x), sin(f_1 y), sin(f_1 z)), \\
%                  &(cos(f_1 x), cos(f_1 y), cos(f_1 z)), \\
%                  & … \\
%                  &(sin(f_L x), sin(f_L y), sin(f_L z)), \\
%                  &(cos(f_L x), cos(f_L y), cos(f_L z))] \in \mathbb{R}^{(2 \times L) \times 3}
% \end{align*}
% Given $2 \times L$ values for sinusoidal encodings of $(x, y, z)$, we trilinearly interpolate into $2 \times L$ number of 3D feature volumes $\mathbf{V} = \{V^{sin}_1, … V^{cos}_L \}$ with each volume shapes as $C \times Q^3$ of channel size $C$ and voxel resolution $Q$.



% The resulting feature vector of length $F = 2 \times L \times C$, is passed into a shallow MLP $f_{\btheta}$ to regress density and geometric features, which are appended with encoded viewing direction to regress color. 

\input{figures/comparison_web}

\input{figures/qualitative}

\subsection{Factorized Plenoptic PNG}
\label{ssec:ppng-12}
% The number of parameters in PPNG-3 is $(F \times Q^3) + \|\theta\|$, where Q represents quantization of 3D feature volume. This makes it hard to reduce the model size without significantly sacrificing quality by reducing Q. 

The vanilla Plenoptic PNG (denoted as PPNG-3) stores a dense 3D volume $\mathbf{V}_i^\mathrm{sin} \in \mathbb{R}^{Q^3 \times D}$ for each frequency, with memory complexity being $Q^3 \times D$. We note that this Fourier-indexed feature representation is axis-aligned and smooth in its index coordinates (sinusoidal space). 
Inspired by the success of tensorial factorization in spatial fields~\cite{Chen2022TensoRFTR}, we  propose leveraging low-rank tensor decomposition techniques to further compress Plenoptic PNG.

Our first approach, PPNG-1, inspired by CP-decomposition~\cite{Chen2022TensoRFTR}, decomposes 3D volumes into a set of triplets of 1D vectors $(\mathbf{v}^r_x, \mathbf{v}^r_z, \mathbf{v}^r_y)$. Specifically, for each $\mathbf{V}_i$ (omitting $\mathrm{sin}$ and $\mathrm{cos}$ superscripts for simplicity), we approximate them using the following equation, instead of directly storing the 3D volume:
\begin{equation}
    \mathbf{V}_i = \sum_r^R
    \mathbf{v}_{i, x}^r \otimes \mathbf{v}_{i, y}^r \otimes  \mathbf{v}_{i, z}^r
    \label{eq:ppng_1_to_3} \text{\ \ (PPNG-1)},
\end{equation}
where $\otimes$ is the outer product, $R$ is the total number of triplet components. PPNG-1 has a memory complexity being $Q\times 3\times R \times D$ for each volume and offers the most compressed representation among all variants with some trade-off in training speed and quality. 


Our second approach, PPNG-2, incorporates tri-plane decomposition to approximate 3D volumes into a set of triplets of 2D feature planes $(\mathbf{v}_{xy}, \mathbf{v}_{xz}, \mathbf{v}_{yz})$:
\begin{equation}
\label{eq:ppng_2_to_3} 
\mathbf{V}_i =
\sum_r^R \mathbf{v}_{i, xy}^r \otimes \mathbf{v}_{i, xz}^r \otimes \mathbf{v}_{i, yz}^r
\text{\ \ (PPNG-2)},
\end{equation}
PPNG-2's memory complexity is $Q^2 \times 3 \times R \times D$ for each volume. It offers a good balance between quality and model size, positioned between PPNG-1 and PPNG-3.

During inference, decoding PPNG-1 and PPNG-2 into the PPNG-3 tensor and loading them into the renderer takes $\mathbb{O}(Q^3 \times R)$ time and can be easily parallelized, making the decoding efficient. Figure~\ref{fig:ppng_1_2} depicts the two representations for one single volume. 


\subsection{Encoding and Implementation Details}
\label{ssec:training}

During the training/encoding stage, given a collection of posed images, we jointly train our Fourier feature volume $\mathbf{V}$ 
and our shallow MLP network $f_\theta$ with volume rendering. We minimize Huber-loss between the volume-rendered pixel colors and observed pixel colors for its robustness to outliers. 

We set volume quantization size $Q=80$, \# of factorized components $R=8$ for PPNG-1, \# of factorized components $R=2$ for PPNG-2, \# of frequency levels $L=4$ and feature dimension $D=4$ throughout all implementations. 
We implement PPNG-1, 2 and 3 in \textit{tiny-cuda-nn}~\cite{Mller2022tinycudann}, which supports voxel-based density caching~\cite{Mller2022InstantNG} for accelerated ray integration. 


The input to our MLP is a feature vector of size $F= 32 = 2 \times L \times C$. A single linear layer produces a density value and a 15-length feature vector.  These values and the degree three spherical harmonics (length 16) of the viewing direction are input to a 2-layer MLP that outputs RGB color and contains a size 16 hidden layer.  In total, our MLP contains 1,072 parameters.  Our experiments ablate using different sized networks.

With the chosen parameters, we have parameter size of $125 KB$ for PPNG-1, $2.45 MB$ for PPNG-2 and $32.7 MB$ for PPNG-3 using half-precision floating points (including shallow MLP weights). 
We encode voxel-based density cache using run-length encoding~(RLE). This typically results in $50 KB$ to $150 KB$ depending on the complexity of the scene. 
We use CBOR~\cite{Bormann2013ConciseBO} to aggregate the Fourier feature parameters, shallow MLP weights, and the voxel-based density caches into a single binary file. We emphasize that all three approaches are directly encoded end-to-end and there are {no additional processes} (a.k.a baking) in converting the optimized PPNG into a binary encoding. 


\input{tables/quantitative}

\subsection{Real-time, Interactive and Portable Viewing}
\label{ssec:rendering}

We visualize PPNG representations in real-time by porting the volume rendering of PPNG in a traditional GL pipeline using WebGL2 with GLSL. Figure~\ref{fig:rendering} illustrates this process. 
Given a binary PPNG file, our decoder first checks which PPNG type (among PPNG-1, 2, and 3) that the binary file contains. If the given binary is PPNG-1 or PPNG-2, we efficiently convert it to PPNG-3 using Eq~\ref{eq:ppng_1_to_3} or Eq~\ref{eq:ppng_2_to_3} respectively. The conversion is parallelized with GLSL-based code. 

Given PPNG-3, we load each volumetric Fourier feature $V$ as a 3D texture image. Since we set $D = 4$, we can use a texture format set as RGBA to load each volume into a single 3D texture image. We set the texture filtering parameter set to linear, which enables tri-linear interpolation for texture sampling the loaded volumes in GLSL.  
We then load RLE encoded voxel-based density cache for empty-space skipping, by decoding it as occupancy grid. 
Similar to the volumetric Fourier feature volumes, we load the occupancy grid as another single-channel 3D texture image. 
Finally, we load shallow MLP by chunking the MLP into set of 4x4 matrices (\texttt{Mat4}) for faster inference. 

At render time, we use a fragment shader to perform volume rendering. From the camera origin, we cast a ray to each pixel in world space, and densely sample along the ray. For each sample, we check if it is occupied with the occupancy grid. If occupied, we query density and color at the sampled point using the method described in Section~\ref{ssec:ppng}. The sampled color and density are integrated with volume rendering equation~\cite{Mildenhall2020NeRFRS} and are terminated if accumulated transmittance falls below a threshold. 
We include a GLSL implementation in the supplementary material. % \jae{leaving mark for supp.}

==> tex/method_bk.tex <==
\input{tex/method_12_bk}
\input{tex/method_34}


==> tex/method_rewrite.tex <==
\section{Plenoptic PNG}
The goal of PPNG is to encode a set of images with known poses into a small model that can be efficiently transmitted and rendered on ubiquitous devices. To achieve this, we first formulate a representation (PPNG-3) that can be rendered efficiently and then formulate factorized representations (PPNG-1, PPNG-2) that are more compact, directly trainable, and efficiently composable after transmission into PPNG-3 for rendering. We implement the models in \textit{tiny-cuda-nn} to support fast training using a voxel-based density cache~\cite{Mller2022InstantNG}, and provide GLSL based code to decode the weights for real-time rendering. 

\subsection{3D Radiance Field Representation with PPNG-3}
\label{ssec:ppng-3}
Our PPNG-3 representation (Figure~\ref{fig:ppng3}) draws insight from the multi-resolution sinusoidal design of positional encoding functions~\cite{tancik2020_fourier}. But, rather than inputting the encodings vectors into a many-layer network, we use them to interpolate into multi-resolution periodic feature volumes, and the resulting feature vector is input into a shallow MLP $f_{\btheta}$. Compared to deep MLPs, the feature volumes are faster to train, and the feature interpolation and shallow MLP are efficiently performed using standard web-based libraries. 

PPNG-3 encodes query point $\mathbf{p}=(x, y, z) \in \mathbb{R}^3$ as :
\begin{align*}
    \gamma(p) = [&(sin(f_1 x), sin(f_1 y), sin(f_1 z)), \\
                 &(cos(f_1 x), cos(f_1 y), cos(f_1 z)), \\
                 & … \\
                 &(sin(f_L x), sin(f_L y), sin(f_L z)), \\
                 &(cos(f_L x), cos(f_L y), cos(f_L z))] \in \mathbb{R}^{(2 \times L) \times 3}
\end{align*}
Given $2 \times L$ values for sinusoidal encodings of $(x, y, z)$, we trilinearly interpolate into $2 \times L$ number of 3D feature volumes $\mathbf{V} = \{V^{sin}_1, … V^{cos}_L \}$ with each volume shapes as $C \times Q^3$ of channel size $C$ and voxel resolution $Q$.



The resulting feature vector of length $F = 2 \times L \times C$, is passed into a shallow MLP $f_{\btheta}$ to regress density and geometric features, which are appended with encoded viewing direction to regress color. 


\input{figures/ppng_1_and_2}
\subsection{Compact Plenoptic Representation with PPNG-1,2}
\label{ssec:ppng-12}
The number of parameters in PPNG-3 is $(F \times Q^3) + \|\theta\|$, where Q represents quantization of 3D feature volume. This makes it hard to reduce the model size without significantly sacrificing quality by reducing Q. Since our volumetric representation is axis aligned, we use volume decomposition techniques to further compress the model size, similar to~\cite{Chen2022TensoRFTR}. 

To compress the 3D feature volume of PPNG-3, we use two types of decomposition: (1) CP-decomposition which decomposes 3D volumes into set of $R_{1}$ triplets of 1D vectors (denoted as PPNG-1), and (2) Tri-plane decomposition which decomposes 3D volumes into set of $R_{2}$ triplets of 2D vectors (denoted as PPNG-2). 

For each volume $V$ in PPNG-3 volumes $\mathbf{V}$ indexed by $(i,j,k)$, we define corresponding CP-decomposed PPNG-1 vectors $v^r_x, v^r_y, v^r_z \in R^{C \times Q}$ with $ 1 \leq r \leq R_1$.
We then, can compose PPNG-3 from PPNG-1 as:
\begin{align*}
    V(i,j,k) = \sum_{1 \leq r \leq R_1} v^r_x(i) \cdot  v^r_y(j) \cdot  v^r_z(k)
\end{align*}
Similarly, we define corresponding tri-plane decomposed PPNG-2 planes $P^r_{xy}, P^r_{yz}, P^r_{xz} \in R^{C\times Q \times Q}$ with $ 1 \leq r \leq R_2$, and compose PPNG-3 as:
\begin{align*}
    V(i,j,k) = \sum_{1 \leq r \leq R_2} P^r_{xy}(i,j) \cdot  P^r_{yz}(j,k) \cdot  P^r_{xz}(i,k)
\end{align*}
Note that computation of PPNG-3 from PPNG-1 and PPNG-2 is trivially parallelizable, each taking compute complexity of $\mathbb{O}(Q^3 \times R_1)$ and $\mathbb{O}(Q^3 \times R_2)$ respectively. 
After decomposition, PPNG-1 compresses PPNG-3 by a factor of $\frac{3 \times R_1}{Q^2}$ and PPNG-2 compresses PPNG-3 by a factor of $\frac{3 \times R_2}{Q}$. 

\subsection{Encoding and Implementation Details}
For training, we implement PPNG-1, 2 and 3 in \textit{tiny-cuda-nn}~\cite{Mller2022tinycudann}, which supports voxel-based density caching~\cite{Mller2022InstantNG} for accelerated ray integration.
We set $Q=80$, $R_1=8$, $R_2=2$, $F=4$ and $C=4$ throughout all implementations. This results in parameter size of $125 KB$ for PPNG-1, $2.45 MB$ for PPNG-2 and $32.7 MB$ for PPNG-3 using half-precision floating points (including shallow MLP weights). 
We encode voxel-based density cache using run-length encoding~(RLE). This typically results in $50 KB$ to $150 KB$ depending on the complexity of the scene. 
We use CBOR~\cite{Bormann2013ConciseBO} to aggregate the parameters, shallow MLP weights and the voxel-based density caches into a single binary file. We emphasize that there are \textbf{no additional processes} (a.k.a baking) in converting the optimized PPNG into a binary encoding. 

\subsection{Real-time Interactive and Portable Viewing}
We visualize PPNG representations in real-time by porting the volume rendering of PPNG in traditional GL pipeline using GLSL. 
We start by loading and converting the data into render-friendly format. 
Initially, PPNG-1 and PPNG-2 are converted into PPNG-3 by parallelized composition as stated in Subsection~\ref{ssec:ppng-12}. 
With PPNG-3, we load feature volumes into 3D textures, with texture sampling set to linear filters. This allows texture sampling done in GLSL to use tri-linear interpolation. 
We then load RLE encoded voxel-based density cache as additional 3D texture after RLE decoding.
Finally, we load shallow MLP by chunking the MLP into set of 4x4 matrices (\texttt{Mat4}). Figure describes this process. 
We volume render PPNG-3 with the loaded textures and matrices by replicating the PPNG-3 rendering process in GLSL (Subsection~\ref{ssec:ppng-3}).
We include a GLSL implementation in the supplementary material. 

==> tex/methods.tex <==
\input{tex/method_12}
\input{tex/method_34}


==> tex/preamble.tex <==
\acmSubmissionID{1069}
\usepackage{booktabs} % For formal tables

% TOG prefers author-name bib system with square brackets
\citestyle{acmauthoryear}

\usepackage[ruled]{algorithm2e} % For algorithms
\usepackage{enumitem}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{tikz}
\usepackage{pifont}
\usepackage[tracking=true]{microtype}
% \usepackage{authblk}
% \usepackage{titling}
\usepackage{listings}
\usepackage{bbding} 
\usepackage{makecell}
\usepackage{multirow}
\usepackage{multicol}
\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\newcommand{\cmark}{\textcolor{darkgreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}%

% Macros
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\btheta}{\bm{\theta}}
\newcommand{\bphi}{\boldsymbol{\phi}}


\renewcommand{\algorithmcfname}{ALGORITHM}
\SetAlFnt{\small}
\SetAlCapFnt{\small}
\SetAlCapNameFnt{\small}
\SetAlCapHSkip{0pt}

% Metadata Information
\acmJournal{TOG}
%\acmVolume{38}
%\acmNumber{4}
%\acmArticle{39}
%\acmYear{2019}
%\acmMonth{7}

% Copyright
%\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
%\setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}

% DOI
%\acmDOI{0000001.0000001_2}

% Paper history
%\received{February 2007}
%\received{March 2009}
%\received[final version]{June 2009}
%\received[accepted]{July 2009}

